SAT Techniques for Lexicographic Path Orders

This seminar report is concerned with expressing LPO-termination of term rewrite systems as a satisfiability problem in propositional logic. After relevant algorithms are explained, experimental results are reported.

==> definitions.tex <==
\lstdefinelanguage{empty}{}
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}

\theoremstyle{definition}
\newtheorem{defi}{Definition}
\newtheorem{ex}{Example}
\newtheorem{rem}{Remark}

\newcommand{\CC}{\mathcal{C}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\VV}{\mathcal{V}}

\newcommand{\lpo}{\succ_{\mathrm{lpo}}}
\newcommand{\qlpo}{\succsim_{\mathrm{lpo}}}
\newcommand{\elpo}{\sim_{\mathrm{lpo}}}
\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}
\newcommand{\remb}{\trianglerighteq_{\mathrm{emb}}}
\newcommand{\premb}{\vartriangleright_{\mathrm{emb}}}
\newcommand{\lemb}{\trianglelefteq_{\mathrm{emb}}}
\newcommand{\plemb}{\vartriangleleft_{\mathrm{emb}}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\F}{\mathsf{F}}
\renewcommand{\t}[1]{\texttt{#1}}
\renewcommand{\rm}[1]{\textrm{#1}}
\newcommand{\m}[1]{\mathsf{#1}}
\newcommand{\limplies}{\rightarrow}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\lex}{\succsim^{\mathrm{lex}}_{\mathrm{lpo}}}
\newcommand{\TTT}{\textsf{T\!\raisebox{-1mm}{T}\!T}}




==> tables/cod_all.tex <==
\begin{table}[bp]
\begin{center}
%\begin{tabular}{|cc|}
%\hline
%strict LPO & quasi LPO \\
%\hline
%  7.89 & 10.26\\
%\hline
%\end{tabular}
\subtable[strict LPO]{
\begin{tabular}{|lcc|}
\hline
        & poSAT & \texttt{SAT}\\
\hline
Total   & 9.112 & 7.666 \\
Average & 0.012 & 0.010 \\
Max     & 0.450 & 0.449 \\
\hline
\end{tabular}
}
\qquad
\subtable[quasi LPO]{
\begin{tabular}{|l r@{.}l r@{.}l |}
\hline
        & \multicolumn{2}{c}{poSAT} & \multicolumn{2}{c|}{\texttt{SAT}}\\
\hline
Total   & 10&428 & 10&690 \\
Average & 0&014 & 0&014 \\
Max     & 1&169 & 0&532 \\
\hline
\end{tabular}
}
\caption{751 instances for poSAT versus 773 instances for \texttt{SAT}.}
\label{RES:cod_all}
\end{center}
\end{table}


==> tables/cod_hard.tex <==

\begin{table}[t]
\renewcommand{\to}{\texttt{TO}}
\begin{center}
\begin{tabular}{|lcccc|}
\hline
TRS & \texttt{SAT} &\texttt{BDD2}& \texttt{BDD3} &\texttt{TTT} \\
\hline
  \sf{AProVE\_AAECC-ring          } & 0.117 &\to  & 0.081      &0.062 \\
  \sf{Cime\_mucrl1                } & 0.296 &0.298& 0.296      &0.932 \\
  \sf{HM\_t005                    } & 0.449 &0.447& 0.449      &\to   \\
  \sf{HM\_t009                    } & 0.123 &\to  & \to        &0.062 \\
  \sf{TRCSR\_Ex1\_2\_AEL03\_C     } & 0.150 &\to  & \it{0.332} &0.121  \\
  \sf{TRCSR\_Ex5\_7\_Luc97\_C     } & 0.117 &\to  & \to        &0.089  \\
  \sf{TRCSR\_Ex6\_15\_AEL02\_C    } & 0.233 &\to  & \it{8.134} &0.171 \\
  \sf{TRCSR\_Ex6\_15\_AEL02\_GM   } & 0.109 &\to  & \to        &0.038  \\
  \sf{TRCSR\_ExAppendixB\_AEL03\_C} & 0.172 &\to  & \it{0.572} &0.151  \\
  \sf{Zantema\_z30                } & 0.091 &0.091& 0.091      &\to   \\
 % TRCSR\_ExSec11\_1\_Luc02a\_C&(0.084)&\to  &\to         &0.075& 0.155 \\
\hline
\end{tabular}
\caption{The 10 hardest problems for the symbol based encoding.}
\label{RES:cod_hard}
\end{center}
\end{table}

